Think in Latent Thoughts: A New Paradigm for Gloss-Free Sign Language Translation

Many SLT systems quietly assume that brief chunks of signing map directly to spoken-language words. That assumption breaks down because signers often create meaning on the fly using context, space, and movement. We revisit SLT and argue that it is mainly a cross-modal reasoning task, not just a straightforward video-to-text conversion. We thus introduce a reasoning-driven SLT framework that uses an ordered sequence of latent thoughts as an explicit middle layer between the video and the generated text. These latent thoughts gradually extract and organize meaning over time. On top of this, we use a plan-then-ground decoding method: the model first decides what it wants to say, and then looks back at the video to find the evidence. This separation improves coherence and faithfulness. We also built and released a new large-scale gloss-free SLT dataset with stronger context dependencies and more realistic meanings. Experiments across several benchmarks show consistent gains over existing gloss-free methods. Our code and data are available at https://github.com/fletcherjiang/SignThought.

==> sec/abs_old.tex <==
% gloss-free 手语翻译（视频→文本），表示现有方法大多是“直接把视频对齐到文本”，缺少“长程语义推理/组合”的机制；我们提出一个可学习的中间推理接口（Cross-Modal Latent Thoughts + Latent CoT） 来做“先思考再生成”，并且发布一个 1300+小时的粤语 HKSL 大规模数据集 LC-HKSLT。
%详细说：这边难点我有了两个词 modality mismatch（模态不匹配）和 information-density mismatch（信息密度不匹配）来表示，后面intro我会详细介绍

\begin{abstract}
Gloss-free Sign Language Translation (SLT) translates sign videos into spoken-language text without gloss supervision, yet remains challenging due to the modality and information-density mismatch between continuous visual-gestural streams and discrete sentences. Most prior methods focus on direct cross-modal mapping, without an explicit mechanism for long-range reasoning and semantic composition.
We take a first step toward reasoning-driven SLT and propose \textbf{\modelname}, which introduces a learnable intermediate reasoning process for gloss-free SLT. \modelname\ uses Cross-Modal Latent Thoughts, a compact set of language-aligned latent states bridging video and text, and a Latent Chain-of-Thought that iteratively refines them with video-conditioned attention, enabling different thoughts to gather evidence from different temporal regions and compose meaning step by step, without intermediate sign supervision. To support research at scale, we also introduce LC-HKSLT, a Cantonese gloss-free SLT dataset with over 1,300 hours of Hong Kong Sign Language videos.
Experiments on five benchmarks show that \modelname\ sets new state of the art, demonstrating latent-thought reasoning as a scalable alternative to gloss supervision that improves accuracy and generalization while reducing annotation cost. Code and data will be released upon acceptance at \url{https://open_upon_acceptance}.
\end{abstract}

% \begin{abstract}
% Gloss-free Sign Language Translation (SLT) aims to translate sign videos into spoken-language text without gloss supervision, but remains difficult due to the severe modality and information-density mismatch between continuous visual-gestural streams and discrete, lexically explicit sentences. Existing gloss-free SLT methods largely treat the task as cross-modal mapping, lacking an explicit mechanism to reason over long-range context and compose higher-level meaning before decoding. 
% In this work, we take the first step toward reasoning-driven SLT and propose \textbf{\modelname}, which explicitly introduces a learnable intermediate reasoning process into gloss-free SLT. \modelname\ introduces Cross-Modal Latent Thoughts, a compact set of language-aligned latent states bridging video and text. A Latent Chain-of-Thought refines them via video-conditioned attention, so different thoughts gather evidence from different temporal regions and compose semantics step by step, without any intermediate sign supervision. To further support research at scale, we introduce LC-HKSLT, a new Cantonese gloss-free SLT dataset with over 1,300 hours of Hong Kong Sign Language videos.
% Extensive experiments on five benchmarks demonstrate that \modelname\ achieves state-of-the-art performance, showing that latent-thought reasoning is a scalable alternative to gloss supervision, which improves accuracy and generalization while substantially reducing annotation costs. Code and data will be released upon acceptance at \url{https://open_upon_acceptance}.
% \end{abstract}

% \begin{abstract}
% Gloss-free Sign Language Translation (SLT) seeks to translate sign videos to text without relying on intermediate sign annotations (glosses), a challenge due to the modality gap between visual-gestural signs and written language. Recent advances have leveraged large language models (LLMs) and visual-language pretraining to bridge this gap. We propose SignCoT, a novel gloss-free SLT model that introduces a Latent Chain-of-Thought architecture to sequentially compose high-level semantic reasoning steps in latent space. Instead of requiring gloss supervision, SignCoT learns a sequence of discrete, language-like latent tokens that progressively capture the meaning of the input signs, effectively bridging the gap between visual and linguistic representations. This chain-of-thought mechanism enables the model to handle complex sign sequences with improved interpretability, as each latent step can be viewed as an implicit reasoning stage. Additionally, we introduce a large-scale Cantonese Sign Language dataset with over 1,300 hours of video. SignCoT achieves state-of-the-art performance across five diverse SLT benchmarks, which are PHOENIX14T, How2Sign, OpenASL, CSL-Daily, and the newly introduced LC-HKSLT (a Hong Kong Sign Language dataset). It outperforms recent top-tier approaches on all metrics. The results demonstrate that composing latent semantic chains without gloss annotations not only reduces costly labeling efforts but also yields more accurate and generalizable translation models, marking a significant step forward in sign language translation. The source code and dataset will be open upon acceptance at \url{https://open_upon_acceptance}.
% \end{abstract}
% \begin{abstract}
%Gloss-free Sign Language Translation (SLT) translates sign videos into spoken-language text without gloss annotations; yet, it remains challenging due to the large modality gap between continuous visual-gestural streams and discrete language. We present \modelname, a gloss-free SLT framework centered on Latent Thoughts, which is a compact sequence of learnable, language-aligned latent states that explicitly support step-by-step semantic composition before generation. \modelname~ introduces a Latent Chain-of-Thought module that iteratively updates latent thoughts through video-conditioned attention, allowing each thought to aggregate evidence from different temporal regions and progressively build higher-level meaning. This yields a gloss-free reasoning interface between vision and language, improving robustness and interpretability without requiring any intermediate sign supervision. 
% Gloss-free Sign Language Translation (SLT) translates sign videos into spoken-language text without gloss annotations, yet remains challenging due to the substantial cross-modal gap between continuous visual-gestural streams and discrete language. We posit that bridging this gap benefits from an explicit intermediate reasoning process before decoding.
% To this end, we propose \textbf{\modelname}, a framework built on Cross-Modal Latent Thoughts: a compact set of learnable, language-aligned latent states that provides an explicit reasoning interface between sign videos and text generation. Building on these thoughts, a Latent Chain-of-Thought module iteratively refines them via video-conditioned attention, allowing different thoughts to aggregate evidence from different temporal regions and progressively compose higher-level semantics step by step, without any intermediate sign supervision.
% %To this end, we propose \textbf{\modelname}, a framework built on \textbf{C}ross-Modal \textbf{La}tent \textbf{T}houghts: a compact set of learnable, language-aligned latent states that provides an explicit reasoning interface between sign videos and text generation. \modelname\ introduces a Latent Chain-of-Thought module that iteratively updates latent thoughts via video-conditioned attention, enabling each thought to route to different temporal evidence and perform step-by-step semantic composition into higher-level meaning. This cross-modal latent thinking paradigm improves robustness and interpretability while requiring no intermediate sign supervision.
% To address the scarcity of large-scale gloss-free SLT corpora, we introduce LC-HKSLT, a new Cantonese SLT dataset with over 1,300 hours of Hong Kong Sign Language videos. Extensive experiments show that \modelname~ achieves state-of-the-art performance across five benchmarks. These results demonstrate that composing translations via latent thoughts is an effective and scalable alternative to gloss supervision, enabling more accurate and generalizable SLT with substantially reduced annotation cost. Code and data will be released upon acceptance at \url{https://open_upon_acceptance}.
% \end{abstract}

==> sec/intro_0102.tex <==
\section{Introduction}
Gloss-Free Sign Language Translation (GF-SLT) aims to directly translate continuous sign language videos into spoken-language text without relying on intermediate gloss annotations. By eliminating costly and labor-intensive gloss supervision~\cite{camgoz2018neural,chen2022two,camgoz2020sign}, GF-SLT offers greater scalability and is particularly promising for low-resource sign languages~\cite{duarte2021how2signlargescalemultimodaldataset,shi2022openasl,uthus2023youtubeasl}. In recent years, advances in end-to-end modeling~\cite{camgoz2018neural,zhou2023gloss,ye2024improvingglossfreesignlanguage,chen2024c2rl} and large pre-trained models~\cite{wong2024sign2gpt,zhou2024scaling,li2025uni} have significantly improved GF-SLT performance. Despite these advances, existing gloss-free approaches still struggle with complex semantic expressions, long-range contextual modeling, and faithful translation, often resulting in missing information, incorrect references, or semantic drift~\cite{voita2018context,cihan2018neural,agarwal2018hallucinations,raunak2021curious,jiao2024visual}.

At a fundamental level, these challenges are not merely caused by modality differences, but closely resemble \textbf{semantic divergence in cross-lingual machine translation.} In multilingual translation, surface-level alignment between source and target forms does not guarantee semantic equivalence due to differences in how meaning is structured and conveyed~\cite{vyas2018identifying}. Similarly, in GF-SLT, the relationship between sign language and spoken language goes far beyond a simple vision-to-text mapping, involving substantial semantic reorganization and contextual dependency~\cite{yin2023gloss,ye2024improvingglossfreesignlanguage}. Treating GF-SLT primarily as a cross-modal alignment or sequence mapping problem therefore provides an incomplete solution.


\begin{figure}[t!]
    \centering
    \includegraphics[width=0.50\textwidth]{latex/Figs/TEASER.png}
    \caption{Comparison Diagram of Different Methods. (\textcolor{red}{Note: just a rough sketch})}
    \label{fig:TEASER}
    \vspace{-1.5em}
\end{figure}

More importantly, from a \textit{\textbf{linguistic perspective}}, \textbf{GF-SLT is not only a mapping problem, but fundamentally a reasoning problem} (Fig.~\ref{fig:TEASER}). Compared to spoken languages, sign languages exhibit sparse explicit lexicalization and rely heavily on implicit cues such as spatial structuring, non-manual signals, and discourse-level context, including referent maintenance and event continuity~\cite{cihan2018neural,li2020tspnet}. As a result, much of the meaning expressed in sign language must be inferred and composed at the discourse level before being realized as surface text. Frame-level or segment-level mapping from video to text tokens is thus linguistically insufficient to support high-quality gloss-free translation.

Reframing GF-SLT as a reasoning problem introduces several fundamental challenges. First, unlike natural language reasoning which operates on discrete symbolic units, GF-SLT inputs consist of high-dimensional continuous visual streams with no explicit semantic boundaries, making it unclear what constitutes valid reasoning primitives. Second, without gloss supervision, existing gloss-free methods lack an explicit intermediate interface for representing and updating semantic state, forcing reasoning to remain implicit within encoder features. Third, faithful translation requires reliable evidence tracking, where generated content can be grounded in corresponding temporal segments of the video; however, current approaches often decode in a largely one-shot manner from dense video features, tightly coupling evidence selection with generation and limiting controllability.

To address these challenges, we propose a \textbf{reasoning-oriented framework} for GF-SLT based on latent thoughts, an explicit intermediate semantic interface between sign videos and text generation. The model first distills the input video into an ordered sequence of latent thoughts that progressively summarize meaning. Building on this representation, we design a plan-then-ground decoding strategy: the model first performs semantic planning by attending to latent thoughts to decide what to say, and then grounds the planned content back to video evidence to decide how to say it, effectively decoupling reasoning from generation.


In summary, our contributions are threefold:

\begin{itemize}
    \item A \textbf{linguistic perspective on gloss-free SLT} is presented, arguing that it is fundamentally a reasoning problem rather than a cross-modal mapping task.
    \item Latent thoughts are introduced as an explicit reasoning-oriented intermediate representation, together with a plan-then-ground decoding framework that separates semantic planning from evidence grounding.
    \item A new large-scale gloss-free SLT dataset is constructed and released, characterized by richer contextual dependencies and realistic semantic expressions, providing a more challenging and practical benchmark for evaluating reasoning-based translation models.
\end{itemize}

==> sec/intro_0105.tex <==
\section{Introduction}
Sign language translation (SLT) is critically important both as a vital assistive technology for connecting Deaf and hard-of-hearing communities and as a challenging multimodal task within natural language processing~\cite{bragg2019interdisciplinary}. 
Research in this area has evolved significantly, progressing from early methods that approached SLT as a gloss-level classification problem over video segments~\cite{koller2015continuous} to more recent formulations as a gloss-free, video-to-text sequence transduction task~\cite{lin2023gloss,chen2024c2rl}, tackled by specialized architectures or multimodal large language models~\cite{wong2024sign2gpt,chen-etal-2024-fla-llm,gong2024signllm}. 
While these efforts have yielded encouraging outcomes, substantial room for improvement remains.

\begin{figure}[htbp]
    \centering
    \includegraphics[width=1\linewidth]{latex/Figs/Fig1.pdf}
    \caption{Latent thoughts provide an explicit intermediate role memory that guides decoding and reduces role reversal in gloss-free SLT}
    \label{fig:introlatent}
\end{figure}
We contend that a fundamental misconception in model design has hindered progress: the treatment of sign video segments as directly mappable to static spoken-language words or phrases~\cite{yin2021including,camgoz2018neural,bragg2019interdisciplinary}. 
This stems from an early narrow focus on the \textit{Frozen Lexicon} (the finite set of conventional signs captured in glossaries), while largely overlooking \textit{Productive Forms}~\cite{forster2014extensions}. 
Productive Forms refer to the other linguistic categorization of signs constructed on-the-fly using classifiers, spatial grammar, and modulation, forming an infinite, context-governed system not captured in gloss lists~\cite{liddell2003grammar}.
For example, a single ``vehicle'' handshape can express meanings like ``park,'' ``crash,'' or ``drive'' through movement variation, obviating the need for separate vocabulary entries~\cite{aronoff2005paradox}. 
Although productive forms constitute a major component of sign language, they have received scant attention in SLT, resulting in models that fail to capture the generative and context-sensitive nature of true sign language semantics~\cite{forster2014extensions,nunez2023survey}.


These linguistic properties indicate that SLT is not a problem of simple symbol substitution or segment-level alignment, but a task that is inherently \textbf{generative and strongly context-dependent}~\cite{yin2021including,bragg2019interdisciplinary}. When productive forms are involved, meaning in sign language is not explicitly encoded by fixed lexical units, but dynamically constructed through motion, spatial configuration, and contextual constraints~\cite{zwitserlood2012classifiers,cormier2012lexicalisation}. As a result, SLT systems must infer, integrate, and abstract latent semantics from sign videos before committing to surface-level text generation, rather than relying on direct mappings from visual patterns to words~\cite{gong2024signllm}.

From this perspective, SLT aligns closely with recent advances in generative reasoning in natural language processing, where models are required to maintain intermediate semantic states and compose meaning under weak or implicit supervision~\cite{wei2022cot,yao2022react}. However, unlike text-only reasoning, reasoning in SLT must operate across visual and linguistic modalities~\cite{mitra2024compositional}. This multimodal nature makes existing reasoning techniques difficult to transfer directly and has left the problem largely underexplored~\cite{yin2021including}. We therefore view this work as a \textit{pilot study} toward understanding how explicit reasoning can be modeled in SLT, with the goal of identifying core challenges and exploring principled solutions~\cite{bragg2019interdisciplinary}.

Specifically, enabling reasoning in SLT poses three key challenges. First, there is a \textbf{\textit{mismatch of reasoning primitives}}: while text reasoning relies on discrete symbolic units, SLT inputs consist of long, continuous visual streams without clear semantic boundaries, making it difficult to structure step-wise inference~\cite{yin2023gloss}. Second, SLT lacks an \textbf{\textit{explicit intermediate reasoning state}}. Most existing models compress semantic information into encoder features, providing no mechanism to represent, update, or query intermediate semantic hypotheses prior to generation~\cite{gong2024signllm}. Third, there is a strong \textbf{\textit{entanglement between reasoning and grounding}}. During generation, the model must both decide what to say and identify the corresponding visual evidence, yet current approaches often conflate these processes, limiting controllability and faithfulness.

To address these challenges, we propose a \textbf{reasoning-oriented framework} for SLT that introduces an explicit intermediate interface between video encoding and text generation. This interface is designed to support structured semantic inference over time, enabling the model to plan content at the semantic level and ground it in visual evidence during generation. By systematically addressing the above challenges, our approach provides a step toward principled multimodal reasoning in sign language translation.

In summary, our contributions are threefold:

\begin{itemize}
    \item A \textbf{linguistic perspective on gloss-free SLT} is presented, arguing that it is fundamentally a reasoning problem rather than a cross-modal mapping task.
    \item Latent thoughts are introduced as an explicit reasoning-oriented intermediate representation, together with a plan-then-ground decoding framework that separates semantic planning from evidence grounding.
    \item A new large-scale gloss-free SLT dataset is constructed and released, characterized by richer contextual dependencies and realistic semantic expressions, providing a more challenging and practical benchmark for evaluating reasoning-based translation models.
\end{itemize}


==> sec/intro_old.tex <==
\section{Introduction}
% 这里先说手语视频翻译到口语文本 对无障碍很关键，但难点来自于连续视觉手势流 vs 离散语言 的跨模态差距。
% 主流 SLT 常用 gloss 作为中间监督，它能给出“按手语顺序的离散标签”，让对齐和解码更容易。
% 但 gloss 成本高、难规模化，而且“gloss bottleneck”可能丢信息、覆盖不足，尤其低资源手语更严重，于是引出 gloss-free SLT 的需求（直接 video→text 训练）。
% 近年 gloss-free 主要靠大模型两条路 （1）借助 LLM/大语言模型：先把手语视频变得更“像语言”（离散 token、分解式训练等），再用 LLM 译文。（2）不直接用 LLM 解码、但强化视觉-语义对齐：比如注意力伪分割、VLP/预训练对齐等。
Translating sign language videos into spoken-language text is essential for accessibility, yet remains challenging due to the cross-modal gap between continuous visual-gestural streams and discrete language. Many SLT systems rely on intermediate gloss annotations~\cite{chen2022two,camgoz2020sign}, which provide sign-ordered supervision and greatly ease alignment and decoding. However, glossing is expensive and hard to scale, and the gloss bottleneck may discard information and limit coverage, especially for low-resource sign languages with scarce annotations~\cite{chen-etal-2024-fla-llm,ye2024improvingglossfreesignlanguage}. These limitations have driven growing interest in gloss-free SLT, which learns direct video-to-text translation without gloss supervision. Recent progress is largely powered by large pre-trained language or multimodal models: some works leverage LLMs by mapping sign videos into more language-like representations (e.g., discrete tokens or factorized training) and then decoding with the LLM~\cite{gong2024signllm,wong2024sign2gpt,chen-etal-2024-fla-llm}, while others improve translation via stronger visual-semantic alignment without explicit LLM decoding, such as attention based pseudo-segmentation or VLP-style pretraining~\cite{yin2023gloss,ye2024improvingglossfreesignlanguage}.

% A linguistic view: SLT is not only mapping, but reasoning.
% 强调一个“语言学事实”（这里也是魏老师要求的，从语言学出发）
% 手语到文本不是“帧→词”映射，而是上下文推理 + 语义组合，真实手语里很多语法或者篇章信息是 隐式表达 的（空间结构等等），不会像口语那样用显式虚词和固定语序写出来。
A key but often under-emphasized linguistic fact is that sign-to-text translation is not a one-shot ``frame-to-word'' mapping. In many real sign languages, crucial grammatical and discourse information is expressed implicitly through spatial structure, non-manual cues, and context-dependent reference tracking (e.g., loci, agreement, entity maintenance), rather than being spelled out as explicit function words and fixed word order in the target sentence~\cite{yin2023gloss}. As a result, producing a fluent spoken-language sentence frequently requires contextual reasoning: maintaining and updating discourse state across time, resolving underspecified references, and composing higher-level meaning before committing to surface lexical choices. This makes gloss-free SLT fundamentally a reasoning-and-generation problem under weak supervision, rather than merely a cross-modal embedding alignment problem.

% Why introducing reasoning into SLT is hard.
% 为什么“把推理引入 gloss-free SLT”很难
% 1. 密度/推理原语不匹配：NLP 推理有天然的离散 token 作推理单元，SLT 输入是上百帧连续信号，没有明确语义边界；没有 gloss 就缺少可用的“语言式原语”来做分步组合，也难把推理过程锚定到视频证据。
% 2. 缺少显式的上下文/状态表示：手语很多意义依赖全局上下文与跨时间的实体关系维护；现有 gloss-free 往往把信息压到 encoder feature 里，让 decoder “自己悟”，缺少一个可更新、可承载中间语义状态的接口。
% 3. 证据跟踪（evidence tracking）与忠实生成（faithful translation）：生成每个片段时必须检索到正确的时间证据，现有“一口气从 dense stream 解码”的证据选择结构弱、难控，容易影响 faithful translation。这里我具体讲一下里面用的evidence tracking什么意思：
% 可以简单理解这个证据就是证视频里支持某个语义或者词的那段时间片段（几帧到几秒）。所以证据追踪就是，这句话的关键信息分别来自视频的哪段，同一个实体/动作在后面再次被提到时，能回到同一证据或相关证据，而不是随便看一眼。
% faithful translation就是我们的翻译严格忠实于源视频表达的内容，不凭空添加、不遗漏关键意思、也不把对象/时间/因果关系翻错。
Reasoning has been extensively studied in NLP, especially with large language models, where evidence, intermediate steps, and outputs reside in a homogeneous symbolic space. In contrast, gloss-free SLT must reason over long, continuous visual signals while generating discrete text, under only sentence-level supervision. This setting introduces three core challenges: \textbf{Density and primitive mismatch.} Text reasoning relies on discrete tokens/sentences that already define stable reasoning primitives and weak alignment cues. For SLT, the input consists of hundreds of frames with no explicit semantic boundaries, whereas the target sentence is lexically explicit and information-dense. Without glosses, there is no readily available set of language-like primitives to support step-wise semantic composition and to anchor a reasoning trace to video evidence.
\textbf{Explicit context/state representation.} Many meanings in signing depend on global discourse and accumulated context (e.g., maintaining entities and relations across time)~\cite{yin2023gloss}. Current gloss-free models typically compress everything into dense encoder features and hope the decoder ``figures it out'', offering no explicit interface for representing and updating intermediate semantic state.
\textbf{Evidence tracking for faithful generation.} Reasoning in SLT is inseparable from grounding: when generating each part of the sentence, the model must retrieve the correct temporal evidence, even under reordering, merging, or omission between signing and text. Existing approaches often decode in a largely one-shot manner from dense encoder streams, where evidence selection over long videos is weakly structured and hard to control, which can reduce faithfulness.

%Our approach: latent thoughts as a reasoning interface.}
% 我们提出方法：latent thoughts + plan-then-ground
% 用 有序的 K 个 latent thoughts 作为 video 和 text 之间的“语言对齐的中间推理接口，不再直接从 encoder feature 翻译，而是先把视频“蒸馏”为一条 thought chain（逐步总结意义）。解码器采用 双流 plan-then-ground：1. 先看 thought chain 决定 what to say（语义规划、全局上下文）；2. 再回看视频 feature 决定 how to say it（证据校验、落地到 token 级内容）。
To address these challenges, we propose \modelname, a framework that explicitly introduces reasoning into gloss-free SLT via an ordered set of $K$ latent thoughts, a compact, language-aligned intermediate interface between video evidence and text generation. Instead of translating directly from dense encoder features, our model first distills the sign clip into a chain of latent thought states that progressively summarize meaning. A dual-stream decoder then follows a plan-then-ground strategy: it first attends to the thought chain to decide \emph{what to say} (semantic planning with global context), and subsequently attends back to the video features to decide \emph{how to say it} with grounded evidence. Crucially, the thought chain is learned end-to-end from video-text pairs and remains fully latent, avoiding the need for gloss supervision. In summary, our contributions are as follows:
% \begin{itemize}
%     \item We reframe gloss-free SLT as a context-dependent semantic reasoning problem under a modality and density mismatch, and introduce an ordered latent-thought interface that provides language-like reasoning primitives for step-wise semantic composition.
%     \item We design a plan-then-ground dual-stream decoder that separates semantic planning (attending to thoughts) from visual grounding (attending to video evidence), improving context utilization and evidence tracking in generation.
%     \item Our approach achieves state-of-the-art performance on multiple SLT benchmarks, and we release LC‑HKSLT, a large‑scale HKSL dataset.
% \end{itemize}
\begin{itemize}
    \item We introduce an ordered set of $K$ learnable latent thought vectors as an explicit intermediate layer between video encoding and text decoding. These thoughts are updated through stacked ThinkingLayers that combine causal self-attention over thoughts to enforce step-wise dependency and cross-attention from thoughts to the encoded sign sequence, allowing for the retrieval of temporally localized evidence. This yields a compact, language-aligned reasoning state without gloss supervision.


    \item We design a decoder that factorizes generation into two complementary attentions at each layer: a planning stream that attends to latent thoughts to determine what to say next, and a grounding stream that attends to the video features to verify and refine token-level content.

    \item Our approach achieves state-of-the-art performance on multiple SLT benchmarks, and we release LC‑HKSLT, a large‑scale HKSL dataset.
\end{itemize}

% \section{Introduction}
% Translating sign language videos into spoken-language text is essential for accessibility, yet remains challenging due to the large modality gap and limited labeled data. Many SLT systems rely on intermediate gloss annotations~\cite{chen2022two,camgoz2020sign}, but glossing is expensive and hard to scale, and the gloss bottleneck may discard information, especially problematic for low-resource sign languages with scarce annotations~\cite{chen-etal-2024-fla-llm,ye2024improvingglossfreesignlanguage}. These limitations have recently driven growing interest in gloss-free SLT, which learns direct video-to-text translation without gloss supervision. In the past two years, gloss-free SLT has progressed rapidly, largely driven by large pre-trained language/multimodal models. Recent methods either leverage LLMs by mapping sign videos into more language-like representations (e.g., discrete tokens or factorized training) and then decoding with the LLM~\cite{gong2024signllm,wong2024sign2gpt,chen-etal-2024-fla-llm}, or improve translation via stronger visual-semantic alignment without explicit LLM decoding, such as attention-based pseudo-segmentation or VLP-style pretraining~\cite{yin2023gloss,ye2024improvingglossfreesignlanguage}.


% % In the past two years, gloss-free SLT has advanced rapidly, with many methods benefiting from large pre-trained language or multimodal models. Representative works integrate an LLM by first producing more “language-like” sign representations (e.g., via discrete tokens or factorized training) and then leveraging the LLM’s strong text prior for translation, leading to consistent gains on standard benchmarks~\cite{gong2024signllm,wong2024sign2gpt,chen-etal-2024-fla-llm}. In parallel, other approaches enhance gloss-free SLT by strengthening visual–semantic alignment without relying directly on LLM decoding. For instance, GASLT mimics the segmentation role of glosses through attention-based mechanisms, encouraging semantically coherent temporal regions, while VLP-style methods inject language priors via large-scale multimodal pretraining to better align sign video features with text semantics~\cite{yin2023gloss,ye2024improvingglossfreesignlanguage}.

% Despite these advances, bringing ``reasoning'' into gloss-free SLT is far from a straightforward transplant from NLP.  Classic reasoning paradigms are typically defined over homogeneous symbolic sequences, where both the evidence and intermediate steps live in the same textual space. In contrast, gloss-free SLT must reason over continuous visual-gestural signals while producing discrete text, under only sentence-level supervision.  This mismatch raises three core challenges. \textbf{(1) Lack of aligned reasoning primitives.} Text reasoning operates over tokens/sentences that already provide discrete units and weak alignment cues. 
% For SLT, the input is a long sequence of frames with no explicit semantic boundaries. 
% Without glosses, there is no readily available set of language-like primitives that a model can use as a stable basis for step-wise semantic composition, making it difficult to form a reliable ``reasoning trace'' anchored to the input evidence. \textbf{(2) Context representation beyond local evidence.} Sign meaning is often context-dependent and discourse-driven: spatial loci, agreement, and entity tracking require maintaining global state across time before committing to surface words. 
% However, current gloss-free models typically encode context implicitly in dense visual features, offering no explicit interface for representing and updating intermediate semantic states that connect local cues to global discourse meaning. \textbf{(3) Evidence tracking for faithful generation.} Reasoning for SLT is inseparable from \emph{grounding}: when generating each part of the sentence, the model must retrieve and justify content with the correct temporal evidence, even under reordering, merging, or omission between signing and text.  Existing approaches often decode in a largely one-shot manner from dense encoder streams, where evidence selection is weakly structured and hard to control, which can lead to unstable long-range dependencies and reduced faithfulness.

% % Despite these advances, gloss-free SLT still faces a fundamental difficulty: translation is not a single-step mapping from frames to words, but a structured semantic composition process. A sign clip typically contains implicit temporal units(phrases/events) without explicit boundaries, many-to-many correspondences between continuous signing and discrete text where content may be reordered, merged, or omitted, and context-dependent meaning (e.g., spatial referencing, agreement, and discourse entities) that requires maintaining and updating intermediate concepts before committing to surface words. Without gloss supervision, most models must recover these latent semantic units and their ordering purely from sentence-level loss. In practice, current approaches often depend on massive pretraining or indirect constraints (token alignment, soft segmentation, or stronger decoders), but they still decode from dense visual streams in a largely ``one-shot'' fashion: intermediate semantic steps are not explicitly represented, and evidence selection over the long video is weakly structured. This makes it hard to reliably bridge long-range dependencies and to produce faithful translations when fine-grained cues must be interpreted under a global context.
% To address these challenges, we propose \modelname, a framework that introduces an ordered set of $K$ latent thoughts as an explicit semantic interface between video evidence and text generation. Instead of translating directly from dense encoder features, our model first distills the sign clip into a chain of latent thought states that progressively summarize meaning, and then decodes with a plan-then-ground strategy: the decoder first attends to latent thoughts to decide what to say, and subsequently attends back to the video features to decide how to say it with grounded evidence. Crucially, these thoughts are learned end-to-end from video-text pairs and remain fully latent, avoiding the need for gloss supervision. The main contributions of \modelname~ are as follows:
% \begin{itemize}
% \item We formulate gloss-free SLT with an ordered latent-thought interface that provides language-like reasoning primitives, enabling step-wise semantic planning from continuous sign signals.
% \item We design a plan-then-ground dual-stream decoder that separates semantic planning (attending to thoughts) from visual grounding (attending to video evidence), improving context utilization and evidence tracking in generation.
% \item Our approach achieves state-of-the-art performance on multiple SLT benchmarks, including PHOENIX14T, How2Sign, OpenASL, CSL-Daily, and our LC-HKSLT dataset.
% \end{itemize}


% % Motivated by the effectiveness of Chain-of-Thought (CoT) reasoning in text models, we ask: \emph{can gloss-free SLT benefit from an explicit, step-wise semantic planning process, while remaining fully latent and end-to-end trainable?} 
% % We propose \textbf{SignCoT}, a Latent Chain-of-Thought architecture for gloss-free SLT. Instead of translating directly from dense encoder features, SignCoT first distills the sign video into an ordered sequence of latent thought states that progressively summarize the semantics of the clip. A dual-stream decoder then follows a plan-then-ground strategy: it first attends to the thought chain to decide what to express, and subsequently attends back to the video features to retrieve how to realize the planned content in fluent text. This design makes the intermediate semantic composition explicit (though latent), providing a structured interface between visual evidence and language generation. The main contributions of SignCoT are as follows:
% % \begin{itemize}
% % \item We introduce a \emph{latent} Chain-of-Thought mechanism for gloss-free SLT, enabling step-wise semantic planning before generation.
% % \item The proposed encoder-thinking-decoder framework learns directly from video-text pairs without gloss annotations, thereby improving scalability in low-resource settings.
% % \item SignCoT achieves state-of-the-art performance on multiple SLT benchmarks, including PHOENIX14T, How2Sign, OpenASL, CSL-Daily, and our LC-HKSLT dataset.
% % \end{itemize}


% %This confers a form of temporal-semantic compositionality: the first few latent tokens might correspond to the subject of the sentence, the next tokens to an action, and so on, mirroring how a gloss sequence or an English sentence is structured, but without any explicit gloss labels. We achieve this by integrating a discrete latent vocabulary learning mechanism, whereby each latent “thought” is chosen from a learned codebook of semantic units. These latent units act as language-like representations of the sign content, effectively serving as an intermediate pseudo-language. The chain-of-thought is thus analogous to an internal caption or explanation for the video, which the text decoder can easily translate into fluent output. Importantly, the entire SignCoT model is optimized end-to-end with only video-sentence pairs, using cross-entropy and latent reconstruction losses, without any gloss-level supervision.




% % Bibliography entries for the entire Anthology, followed by custom entries
% %\bibliography{anthology,custom}
% % Custom bibliography entries only
% \begin{table*}[t]
% \centering
% \resizebox{1\linewidth}{!}{\begin{tabular}{l|c|c|c|c|c|c|c}
% \toprule
% Dataset / Work & Lang. & SLR Vocab. & SLT Vocab. & Duration (h) & Videos & Signers & Source \\
% \midrule
% GSL~\cite{adaloglou2021comprehensive}                 & GSL      & 310    & --      & 9.59 & 10K   & 7  & Lab \\
% PHOENIX\textendash 14T \cite{camgoz2018neural}   & DGS      & 1{,}066& 2{,}887  & 10.53 & 8K    & 9  & TV  \\
% CSL\textendash Daily \cite{zhou2021improving}   & CSL      & 2{,}000& 2{,}370 & 23.27 & 21K   & 10 & Lab \\
% TVB\textendash HKSL\textendash News \cite{niu2024hongkongsignlanguage} & HKSL & 6{,}515 & 2{,}850 & 16.07& 7K & 2 & TV \\
% \midrule
% \textbf{LC\textendash HKSLT (Ours)} & HKSL     & --     & 125{,}833 & 1311& 432K & 14 & YouTube \\
% \bottomrule
% \end{tabular}}
% \caption{Comparison of LC\textendash HKSLT with representative SLR/SLT datasets.}
% \label{tab:hk_dataset_compare}
% \end{table*}






==> sec/method_new.tex <==
\section{Problem Formulation}\label{sec:reasoning_formulation}

% \paragraph{Task Definition and Supervision Regime.}
This work studies the problem of gloss-free sign language translation (SLT). Given an input sign language video$V = \{v_t\}_{t=1}^{T}$ consisting of $T$ visual frames,the goal is to generate a spoken-language sentence$Y = \{y_n\}_{n=1}^{N}$.Unlike gloss-based approaches, no intermediate gloss annotations or temporal supervision are available. The model is trained solely with sentence-level video--text pairs $(V, Y)$, without explicit supervision on alignments, segmentations, or intermediate semantic structures. This setting requires the model to internally organize frame-level visual evidence and infer high-level semantic abstractions that can reliably support translation under weak supervision.

% \paragraph{Budgeted Cross-modal Latent Reasoning Formulation.}
Rather than treating gloss-free SLT as a direct sequence-to-sequence mapping, we formulate it as a budgeted cross-modal latent reasoning problem. We posit that accurate translation is mediated by a small set of intermediate semantic states that organize visual evidence before lexical decisions are made.Formally, we introduce an ordered latent variable$C = \{c_k\}_{k=1}^{K}$,where each $c_k$ denotes a latent thought state.The number of latent thoughts $K$ is explicitly bounded, representing a constrained reasoning budget. These latent thoughts are neither textual tokens nor predefined linguistic units; instead, they constitute cross-modal semantic states that bridge visual perception and language generation.R easoning is modeled as an iterative inference process over $C$, where the latent thoughts are progressively refined by selectively incorporating visual evidence over a fixed number of steps $L$, forming a finite-horizon reasoning trajectory in latent space. The final translation $Y$ is generated by conditioning the decoder on the inferred latent thoughts, which serve as a structured and interpretable semantic interface between perception and language.


\subsection{Budgeted Latent Thought Reasoning over Visual Evidence} \label{sec:latent_reasoning}
Given the formulation in Section~\ref{sec:reasoning_formulation}, we instantiate budgeted cross-modal reasoning as an explicit latent inference process operating over visual evidence. The input video $V$ is first encoded into a sequence of frame-level features $E = \{e_t\}_{t=1}^{T}$, which serve solely as perceptual evidence. Crucially, these features do not directly drive language generation; instead, all translation decisions are mediated through a set of latent thought states, ensuring a clear separation between evidence acquisition and semantic reasoning. 

We maintain an ordered set of latent thoughts $C = \{c_k\}_{k=1}^{K}$, where $K$ is a fixed reasoning budget. At initialization, the thoughts form a set of learnable reasoning states that do not correspond to predefined tokens or linguistic units. This design enforces a bounded semantic workspace, within which the model must organize and abstract visual evidence. By constraining the number of thoughts, the reasoning process is encouraged to capture salient and complementary semantic hypotheses, rather than distributing information across unconstrained latent dimensions. 

Reasoning proceeds through an iterative refinement process over a fixed horizon of $L$ steps. At each step $\ell \in \{1, \ldots, L\}$, the latent thoughts $C^{(\ell)}$ are updated by selectively incorporating information from $E$, conditioned on their current states. This iterative update defines a finite-horizon trajectory $\{C^{(0)}, C^{(1)}, \ldots, C^{(L)}\}$ in latent space, which can be interpreted as a sequence of intermediate reasoning states. Importantly, no textual tokens are generated during this process; all intermediate computation remains non-textual and latent, distinguishing it from open-ended chain-of-thought decoding. 

The ordering of latent thoughts is preserved throughout the reasoning process, endowing the latent space with an implicit structural bias. Rather than treating the thoughts as an unordered memory bank, the model learns to distribute semantic responsibilities across ordered reasoning slots, allowing different thoughts to focus on distinct aspects of the input video. This ordered structure supports compositional reasoning, where higher-level semantics emerge from the coordinated evolution of multiple latent states under a fixed budget. 

From a computational perspective, the iterative refinement of latent thoughts can be viewed as a constrained rollout in latent space. The reasoning horizon $L$ and thought budget $K$ jointly define the computational and representational limits of the reasoning process. Unlike textual rollouts that rely on stochastic decoding, this latent rollout is deterministic conditioned on the input and governed by learned update rules. As a result, the reasoning trajectory is stable, bounded, and amenable to analysis. 

By design, the final latent thoughts $C^{(L)}$ constitute a structured semantic interface between visual perception and language generation. They summarize the input video at a level of abstraction suitable for downstream decoding, while retaining explicit links to the underlying visual evidence. Subsequent stages operate exclusively on these inferred thoughts, ensuring that translation decisions are grounded in the outcome of the constrained latent reasoning process, rather than direct frame-level correlations. 


\subsection{Constrained Evidence Routing and Traceable Thought Assignment}
\label{sec:routing_traceability}

While the latent thought reasoning process described in Section~\ref{sec:latent_reasoning} defines how intermediate semantic states evolve, it does not by itself specify how visual evidence is distributed across thoughts. To ensure that reasoning remains structured and interpretable, we introduce an explicit evidence routing mechanism that assigns visual evidence to latent thoughts under well-defined constraints.  

At each reasoning step $\ell$, we compute a routing matrix $A^{(\ell)} \in \mathbb{R}^{K \times T}$, where each entry $A^{(\ell)}_{k,t}$ quantifies the degree to which the $t$-th frame-level feature $e_t$ contributes to the $k$-th latent thought $c_k$. This routing matrix serves as an explicit responsibility assignment, binding perceptual evidence to semantic reasoning states. Rather than allowing unconstrained attention, we impose structural constraints on $A^{(\ell)}$ to regulate how evidence can be allocated.  Specifically, the routing matrix is normalized to satisfy global assignment constraints, ensuring that evidence allocation across latent thoughts is balanced and well-formed. By enforcing these constraints, the model is discouraged from collapsing all evidence into a single thought or diffusing semantics across redundant states. As a result, each latent thought is encouraged to specialize in a subset of visual evidence, leading to a more interpretable and disentangled reasoning process. The constrained routing mechanism thus plays a dual role: it stabilizes latent reasoning and enforces a meaningful division of semantic labor.  The routing variables $A^{(\ell)}$ are not auxiliary artifacts, but constitute an integral part of the reasoning trajectory. Together with the latent thoughts $C^{(\ell)}$, they define a coupled evolution of \emph{what} semantic hypotheses are formed and \emph{which} visual evidence supports them. This coupling ensures that updates to latent thoughts are grounded in explicit evidence assignments, rather than implicit correlations in latent space.  An important consequence of explicit routing is the traceability of the reasoning process. For any output token generated by the decoder, we can trace its dependency path from the token-level attention over latent thoughts, to the corresponding routing assignments, and ultimately to the contributing video frames. This enables post-hoc inspection of which latent thoughts were responsible for a given decision and which segments of the input video provided the supporting evidence. Such traceability distinguishes our approach from models where intermediate reasoning is embedded in opaque hidden states.  By constraining evidence routing and making thought–evidence assignments explicit, the proposed mechanism transforms latent reasoning from an unstructured internal computation into a structured and analyzable process. This design not only improves interpretability, but also provides a foundation for validating and diagnosing reasoning behavior, as will be further explored in subsequent sections. 



==> sec/method_old.tex <==
\section{LC-HKSLT Dataset}
To study large-scale, gloss-free SLT in a realistic setting, we construct \textbf{LC-HKSLT}, a Hong Kong Sign Language corpus curated from broadcast-style public briefings with continuously visible interpreters.
It contains 1,311 hours (432K clips) and provides only sentence-level supervision (no glosses or SLR vocabularies), matching our intended deployment regime. Full collection details and statistics are provided in Appendix~\ref{app:lchkslt}.



\section{Method}
%目前都超很多字数，这里也超字数了，所以我直接把Problem Formulation这部分注释了
\subsection{Problem Formulation}
We study gloss-free sign language translation (SLT), where the supervision consists solely of sentence-level translations without any intermediate gloss annotations. Given a sign video clip, we aim to generate a target spoken-language sentence. Let a sign clip be represented as a sequence of visual observations
$\mathbf{X}=\{x_t\}_{t=1}^{T_s}$ (e.g., RGB frames or pre-extracted pose/region features).
A binary mask $\mathbf{m}\in\{0,1\}^{T_s}$ indicates valid time steps when clips are padded. The target translation is a token sequence
$\mathbf{Y}=\{y_t\}_{t=1}^{T_t}$ with $y_t\in\mathcal{V}$, where $\mathcal{V}$ is the text vocabulary. We assume a dataset of paired samples
$\mathcal{D}=\{(\mathbf{X}^{(n)}, \mathbf{Y}^{(n)})\}_{n=1}^{N}$.
Crucially, no gloss sequence or sign-token alignment is provided. We learn a conditional sequence model that maximizes the likelihood of the target sentence given the sign clip:
\begin{equation}
p_\theta(\mathbf{Y}\mid \mathbf{X})
=\prod_{t=1}^{T_t} p_\theta\!\left(y_t \mid y_{<t}, \mathbf{X}\right).
\end{equation}
In addition to the standard autoregressive formulation, our method introduces a set of $K$ ordered latent thought states $\mathbf{C}=\{c_k\}_{k=1}^{K}$ that serve as an intermediate semantic plan distilled from $\mathbf{X}$ and consumed by the decoder during generation.


% 一句话说我的们的模型 encoder → thinking → decoder
\subsection{Overall Architecture}
% TODO: zhangli: 建议放pipeline图的caption
As illustrated in Fig.~\ref{fig:pipeline}, the proposed model adopts an encoder thinking decoder architecture. Given an input sign clip $\mathbf{X}$, a sign encoder first extracts contextualized visual representations $\mathbf{E} = \mathrm{Enc}(\mathbf{X})$. A Latent Chain of Thought module subsequently condenses $\mathbf{E}$ into an ordered set of $K$ latent thought states $\mathbf{C} = \mathrm{Think}(\mathbf{E})$, which functions as a compact semantic plan. Conditioned on both the latent thought chain $\mathbf{C}$ and the encoder features $\mathbf{E}$, a dual stream autoregressive decoder then generates the target sentence.


% In the remainder of this section, we describe each component in detail: the sign encoder in Sec.~\ref{sec:encoder}, the Latent CoT thinking module in Sec.~\ref{sec:thinking}, and the dual-stream decoder in Sec.~\ref{sec:decoder}, followed by the training objective and inference procedure.



% 很经典的encoder结构，不多讲了，没什么特别的
\subsection{Sign Encoder}
\label{sec:encoder}
% The encoder maps an input sign clip into a contextualized sequence of visual representations that preserves fine-grained temporal evidence for translation.

Given a sign video clip $\mathbf{X}=\{x_t\}_{t=1}^{T_s}$ (frames or pre-extracted visual/pose features), we maintain a binary mask $\mathbf{m}$ to indicate valid time steps under padding. We first project the raw per-frame features into the model space via a learnable embedding layer:
\begin{equation}
\mathbf{E}^{(0)} = \mathrm{Embed}(\mathbf{X}),
\end{equation}
where $\mathrm{Embed}(\cdot)$ is implemented as a linear projection followed by normalization and dropout. This step unifies heterogeneous sign features into a shared representation space for subsequent sequence modeling.


To inject order information, we add positional encoding to obtain
\begin{equation}
\hat{\mathbf{E}}^{(0)} = \mathbf{E}^{(0)} + \mathrm{PosEnc}(\mathbf{E}^{(0)}),
\end{equation}
with dropout applied afterward. We then stack $N$ encoder layers to model long-range dependencies and local motion patterns:
\begin{equation}
\hat{\mathbf{E}}^{(n)} = \mathrm{EncBlock}^{(n)}(\hat{\mathbf{E}}^{(n-1)}, \mathbf{m}), \quad n=1,\dots,N,
\end{equation}
where each $\mathrm{EncBlock}$ follows a Conformer-style design, combining multi-head self-attention (masked by $\mathbf{m}$) with a lightweight convolutional module to capture local temporal dynamics, together with feed-forward sublayers and residual normalization. The final encoder output is
\begin{equation}
\mathbf{E}=\hat{\mathbf{E}}^{(N)}=\{e_t\}_{t=1}^{T_s}.
\end{equation}

The resulting sequence $\mathbf{E}$ serves as the frame-level evidence source for both the Latent CoT thinking module (Sec.~\ref{sec:thinking}) and the dual-stream decoder (Sec.~\ref{sec:decoder}).



% 核心部分，一句话解释就是把证据压缩成 有序k步语义计划c，并通过a建立 thought和时间段的绑定，相当于就是先把长视频证据整理成一条可控的思考链，再交给 decoder 去写句子。
\subsection{Latent Chain-of-Thought Thinking Module}
\label{sec:thinking}
The objective of the thinking module is to transform the dense encoder representations $\mathbf{E}$ into a compact and ordered set of $K$ latent thought states $\mathbf{C}=\{c_k\}_{k=1}^{K}$, which collectively serve as a high-level semantic plan for translation. In contrast to gloss-based pipelines, these thought states are learned end-to-end under sentence-level supervision and are explicitly organized to form a directional latent chain.

% \paragraph{Inputs and outputs.}
Given encoder features $\mathbf{E}=\{e_t\}_{t=1}^{T_s}$ and the corresponding source mask, the module outputs
\begin{equation}
\mathbf{C} = \mathrm{Think}(\mathbf{E}) \in \mathbb{R}^{K},
\end{equation}
where the index $k$ defines the causal order of the latent reasoning process.

\paragraph{Learnable thought slots.}
A central difficulty in gloss-free SLT is that the video provides dense and redundant evidence, while the translation requires a compact sequence of semantic decisions. Instead of forcing the decoder to discover this structure on the fly, we introduce an explicit intermediate interface: a small set of ordered thought slots that serve as the model’s working memory for step-wise semantic composition.
% Concretely, we maintain $K$ learnable vectors $\mathbf{Q}=\{q_k\}_{k=1}^{K}$, expanded to each mini-batch to form $\mathbf{C}^{(0)}$. 
Concretely, we initialize the thought chain with $K$ learnable slots $\mathbf{C}^{(0)}=\{c_k^{(0)}\}_{k=1}^{K}$, where each $c_k^{(0)}\in\mathbb{R}^{d}$ is a trainable parameter, serving as empty reasoning states before evidence injection. These slots can be viewed as \emph{empty} reasoning states that will be filled with semantic evidence distilled from $\mathbf{E}$.

\paragraph{Thinking layers.}
A key bottleneck in gloss-free SLT is that the encoder produces a long, continuous evidence stream $\mathbf{E}$, while what we ultimately need for generation is a compact and structured semantic plan.
If we let the decoder directly attend to all frames, it must simultaneously decide what to express and where the supporting evidence lies, which often leads to diffuse attention and unstable evidence tracking.
We therefore introduce a dedicated thinking stage that repeatedly compresses and reorganizes $\mathbf{E}$ into an ordered latent chain $\mathbf{C}$ before decoding. To make this compression process expressive yet controllable,
we stack $L$ identical thinking layers to iteratively refine the chain:
\begin{equation}
\mathbf{C}^{(\ell)} = \mathrm{ThinkLayer}^{(\ell)}(\mathbf{C}^{(\ell-1)}, \mathbf{E}), \quad \ell=1,\dots,L,
\end{equation}
and set $\mathbf{C}=\mathbf{C}^{(L)}$ as the final latent chain-of-thought. Each thinking layer consists of two main steps: causal thought mixing to impose an ordered chain prior, and an evidence-routed cross-attention operator that retrieves sign evidence in a structured manner.

% \paragraph{Causal thought mixing.}
We first encourage a directional (coarse-to-fine) refinement inside the latent chain.
Specifically, we apply masked self-attention over the $K$ thought states using a lower-triangular (causal) mask, so that the $k$-th thought only attends to $\{1,\dots,k\}$:
% We apply masked self-attention over the $K$ thought states using a lower-triangular (causal) mask, so that the $k$-th thought only attends to $\{1,\dots,k\}$:
\begin{equation}
\tilde{\mathbf{C}}^{(\ell)} = \mathrm{CausalSelfAttn}\!\left(\mathbf{C}^{(\ell-1)}\right).
\end{equation}
This simple prior turns the thought set into an ordered workspace: earlier thoughts summarize coarse semantics and provide context, while later thoughts refine with additional details, making the intermediate reasoning process more stable and interpretable.
% This enforces a directional refinement process (coarse-to-fine) within the latent chain.

% \paragraph{Evidence-routed cross-attention.}
The second challenge is evidence assignment. A standard cross-attention from thoughts to all frames is both inefficient on long clips and prone to degeneracy, where multiple thoughts attend to the same frames. We address this by routing before retrieval: each thought is first softly bound to a contiguous semantic region (at a coarse level), and only then retrieves fine-grained evidence within that responsibility region.

% Instead of a standard cross-attention from thoughts to all frames, we use a routed evidence operator that constructs a multi-granular evidence fabric from $\mathbf{E}$ and performs soft routing to bind each thought to a contiguous semantic region before retrieval.

% \textbf{Evidence fabric.} 
From the frame-level stream $\mathbf{E}$, we derive (i) frame evidence (the original tokens), (ii) a small set of segment-level tokens $\mathbf{S}$ obtained by a differentiable soft segmentation over time, and (iii) a global summary token $g$ (masked pooling). Intuitively, $\mathbf{S}$ provides sparse semantic ``chunks'' (analogous to latent phrase units) while frame evidence preserves fine-grained lexical details.

% \textbf{Routing and binding.} Given segment tokens $\mathbf{S}$, we compute an affinity between each thought and each segment, and apply a differentiable normalization (Sinkhorn-style) to obtain a soft binding matrix $\mathbf{A}$ that assigns segment evidence to each thought. This produces a routed segment summary for each thought:
% \begin{equation}
% p_k = \sum_j A_{k,j}\, S_j,
% \end{equation}
% where $p_k$ represents the semantic responsibility region of thought $c_k$. We optionally bias the routing to be weakly monotonic in $k$ (coarse-to-fine progression), while keeping the assignment fully soft.
% \textbf{Routing and binding.} 
Given segment tokens $\mathbf{S}=\{S_j\}_{j=1}^{M}$ and latent thoughts $\mathbf{C}=\{c_k\}_{k=1}^{K}$, we compute a similarity score matrix $\mathbf{G}\in\mathbb{R}^{K\times M}$ with
\begin{equation}
G_{k,j} = \frac{(W_q c_k)^\top (W_k S_j)}{\sqrt{d}} .
\end{equation}
We then apply a differentiable Sinkhorn-style normalization to obtain a soft binding matrix
$\mathbf{A}=\mathrm{Sinkhorn}(\mathbf{G})\in\mathbb{R}^{K\times M}$, where $A_{k,j}\ge 0$ denotes the (soft) amount of segment $j$ assigned to thought $k$. In practice, we normalize $\mathbf{A}$ to be approximately doubly stochastic (i.e., rows and columns sum to 1 up to a small error $\epsilon$), which encourages balanced, non-collapsed routing while remaining fully soft.
Each thought receives a routed segment summary:
\begin{equation}
p_k = \sum_{j=1}^{M} A_{k,j}\, S_j,\qquad p_k\in\mathbb{R}^{d},
\end{equation}
where $p_k$ summarizes the segment evidence that thought $c_k$ takes responsibility for. We optionally add a weak monotonic bias over $k$ (coarse-to-fine progression) while keeping $\mathbf{A}$ fully soft.
% \textbf{Routed retrieval.}
Conditioned on the routed summary $p_k$, each thought retrieves fine-grained sign evidence from $\mathbf{E}$ via cross-attention (and optionally sparse/deformable retrieval for efficiency on long clips). We denote the resulting evidence-aware thought update by
\begin{equation}
\hat{\mathbf{C}}^{(\ell)} = \mathrm{RoutedXAttn}\!\left(\tilde{\mathbf{C}}^{(\ell)}, \mathbf{E}\right),
\end{equation}
where $\mathrm{RoutedXAttn}$ encapsulates \emph{(fabric $\rightarrow$ routing $\rightarrow$ retrieval)} as a single operator in our implementation and in the overview figure.

% \paragraph{Layer update.}
Finally, we apply a position-wise feed-forward network with residual normalization to produce the layer output:
\begin{equation}
\mathbf{C}^{(\ell)} = \mathrm{FFN}\!\left(\hat{\mathbf{C}}^{(\ell)}\right).
\end{equation}

% \paragraph{Interface to the decoder.}
The final thought chain $\mathbf{C}$ is consumed by the decoder through thinking cross-attention (Sec.~\ref{sec:decoder}). In addition, the intermediate routing variables (e.g., the thought-to-segment binding $\mathbf{A}$ and the segmentation weights) can be cached as an internal prior to guide visual grounding in the dual-stream decoder, without changing the model Input and Output.


% Dual-Stream Decoder 就是把解码时的生成拆成两步：1. 先用 latent thoughts 做语义规划（决定要说什么），2. 再回到视频特征做视觉校验（决定怎么说、是否忠实）。
\subsection{Dual-Stream Decoder}
\label{sec:decoder}
We adopt an autoregressive Transformer decoder that explicitly follows a \emph{plan-then-ground} generation pattern. 
At each layer, the decoder first consults the latent thought chain to decide \emph{what} semantic content to express, and then returns to the encoder features to retrieve fine-grained signing evidence for \emph{how} to realize that content in fluent text.

% \paragraph{Input embeddings.}
Given an input text prefix $\mathbf{y}_{<t}$ (teacher forcing during training), we embed tokens with standard word and positional (and optionally token-type) embeddings to obtain decoder states.

% \paragraph{Decoder layer.}
Let $\mathbf{H}^{(l-1)}$ denote the decoder hidden states entering layer $l$. Each layer contains the following sub-layers. We first apply masked self-attention over previously generated tokens to produce
\begin{equation}
\mathbf{H}^{(l)}_{\mathrm{self}}=\mathrm{MSA}\!\left(\mathbf{H}^{(l-1)}\right),
\end{equation}
where the subsequent mask ensures autoregressive generation.

We then attend to the latent thought chain $\mathbf{C}$:
\begin{equation}
\mathbf{H}^{(l)}_{\mathrm{think}}=\mathrm{XAttn}\!\left(\mathbf{H}^{(l)}_{\mathrm{self}},\,\mathbf{C}\right).
\end{equation}
Intuitively, this step selects the current semantic ``reasoning state'' from the ordered thoughts, providing a high-level plan for the next tokens. We also retain the corresponding attention weights over thoughts,
denoted by $\boldsymbol{\alpha}$, as they reflect which thought(s) each target position relies on.


To make ``think first, then ground'' a \emph{mechanism} rather than only an ordering, we derive a soft temporal retrieval prior from $\boldsymbol{\alpha}$ using intermediate routing variables cached in the thinking module. Specifically, we reuse (i) the thought-to-segment binding matrix $\mathbf{A}$ (from Sinkhorn routing), and (ii) the segment-to-frame aggregation weights $\mathbf{W}_{seg}$ (from soft segmentation). We map token-to-thought attention to a token-to-frame prior:
\begin{equation}
\boldsymbol{\beta} = \boldsymbol{\alpha}\mathbf{A},\qquad
\mathbf{w} = \boldsymbol{\beta}\mathbf{W}_{seg},
\end{equation}
where $\mathbf{w}$ assigns each target position a soft preference over source time steps. This routing prior is internal (no change to model I/O) and can be omitted without affecting the decoder interface.

Finally, we attend to the encoder features $\mathbf{E}$ to obtain grounded decoder states:
\begin{equation}
\mathbf{H}^{(l)}_{\mathrm{vis}}=\mathrm{XAttn}\!\left(\mathbf{H}^{(l)}_{\mathrm{think}},\,\mathbf{E}\right),
\end{equation}
with the standard source mask applied. When the routing prior $\mathbf{w}$ is enabled, we incorporate it as a soft bias in the attention logits, encouraging the decoder to retrieve evidence from time regions consistent with the selected thought(s). This yields thought-guided evidence retrieval while preserving the standard Transformer decoder structure.

A position-wise FFN with residual connections and layer normalization produces the layer output:
\begin{equation}
\mathbf{H}^{(l)}=\mathrm{FFN}\!\left(\mathbf{H}^{(l)}_{\mathrm{vis}}\right).
\end{equation}



% \paragraph{Output projection.}
The final decoder states are projected to the vocabulary to obtain token probabilities, and the model is trained with the standard sequence-level cross-entropy objective (Sec.~\ref{sec:objective}).


% 损失函数介绍
% 1. 交叉熵，经典的，没特别的
% 2. 单调正则，约束第 k 个 thought 绑定的视频段位置不要跑到第 k+1 个后面去（不要乱序或者到后面去） 相当于就是让 thoughts 按时间顺序推进。
% 3. 连续正则，用 TV 惩罚让每个 thought 关注的 segment 分布更平滑、更像连续一段，而不是东一块西一块。简单说：让每个 thought 对应一段连续证据。
\subsection{Training Objective}
\label{sec:objective}
All components (encoder, thinking module, and decoder) are trained end-to-end with sentence-level supervision. 



\paragraph{Translation loss.}
Given a mini-batch of paired data $\{(\mathbf{X}^{(b)},\mathbf{Y}^{(b)})\}_{b=1}^{B}$, where $B$ is the batch size and $T_t$ is the target length, we train the dual-stream decoder with teacher forcing and standard cross-entropy:
\begin{equation}
\mathcal{L}_{ce}
= -\frac{1}{B}\sum_{b=1}^{B}\sum_{t=1}^{T_t}
\log p_\theta\!\left(y^{(b)}_t \mid y^{(b)}_{<t}, \mathbf{E}^{(b)}, \mathbf{C}^{(b)}\right).
\end{equation}




\paragraph{Latent chain regularization.}
To encourage the latent thoughts to behave as an ordered chain of contiguous semantic units, we add two simple regularizers on the thought-to-segment assignment matrix $\mathbf{A}$ produced by the thinking module (Sec.~\ref{sec:thinking}).

% \textbf{(1) Monotonic progression.}
Let $\mu_k$ be the expected segment index assigned to the $k$-th thought:
\begin{equation}
\mu_k = \sum_{j=1}^{M_{seg}} j \cdot A_{k,j}.
\end{equation}
We penalize violations of the forward (coarse-to-fine) progression:
\begin{equation}
\mathcal{L}_{mono}
= \frac{1}{B}\sum_{b=1}^{B}\sum_{k=1}^{K-1}
\mathrm{ReLU}\!\left(\mu_k-\mu_{k+1}+\delta\right),
\end{equation}
where $\delta$ is a small margin.

% \textbf{(2) Contiguity.}
We encourage each thought to focus on a contiguous region in segment space using a total-variation penalty:
\begin{equation}
\mathcal{L}_{cont}
= \frac{1}{BK}\sum_{b=1}^{B}\sum_{k=1}^{K}\sum_{j=2}^{M_{seg}}
\left|A_{k,j}-A_{k,j-1}\right|.
\end{equation}

\paragraph{Overall objective.}
Our final training loss is:
\begin{equation}
\mathcal{L}_{total}
= \mathcal{L}_{ce}
+ \lambda_{mono}\mathcal{L}_{mono}
+ \lambda_{cont}\mathcal{L}_{cont}
\end{equation}
where $\lambda_{mono}$ and $\lambda_{cont}$ control the strength of structural regularization; we set them to $0.1$ and $0.2$ in all experiments unless otherwise specified.







